Theoretical Analysis of the Radio Map Estimation Problem

Radio maps provide radio frequency metrics, such as the received signal strength, at every location of a geographic area. These maps, which are estimated using a set of measurements collected at multiple positions, find a wide range of applications in wireless communications, including the prediction of coverage holes, network planning, resource allocation, and path planning for mobile robots. Although a vast number of estimators have been proposed, the theoretical understanding of the radio map estimation (RME) problem has not been addressed. The present work aims at filling this gap along two directions. First, the complexity of the set of radio map functions is quantified by means of lower and upper bounds on their spatial variability, which offers valuable insight into the required spatial distribution of measurements and the estimators that can be used. Second, the reconstruction error for power maps in free space is upper bounded for three conventional spatial interpolators. The proximity coefficient, which is a decreasing function of the distance from the transmitters to the mapped region, is proposed to quantify the complexity of the RME problem. Numerical experiments assess the tightness of the obtained bounds and the validity of the main takeaways in complex environments.

==> notation_bf_gamma_change.tex <==

%% parent file: draft.tex
\renewcommand{\define}{\triangleq}
\renewcommand{\expected}{\mathbb{E}}
\newcommand{\spanc}{\overline{\spanv}}
\newcommand{\auxfun}{{\hc{g}}}
\newcommand{\auxset}{{\hc{B}}}
\newcommand{\measure}{{\hc{\mu}}}
\newcommand{\fourier}{\mathcal{F}}
\newcommand{\eigmax}{\hc{\mathcal{\lambda}}_{\text{max}}}
\newcommand{\bw}{{\hc{B}}} % bandwidth

\newcommand{\aconst}{\hc{a}}
\newcommand{\auxvec}{{\hc{\bm v}}} % auxiliary vector
\newcommand{\auxmat}{{\hc{\bm A}}} % auxiliary matrix
\newcommand{\auxmatent}{{\hc{A}}} % auxiliary matrix entry
\newcommand{\auxvar}{{\hc{x}}} % auxiliary variable

\newcommandoa{\mapregion}{\hc{\mathcal{R}}}{\hc{\mathcal{R}}^{(#1)}}
\newcommand{\auxmapregion}{\hc{\tilde{\mathcal{R}}}}
\newcommandoa{\srcregion}{\hc{\mathcal{V}}}{\hc{\mathcal{V}}^{(#1)}}
\newcommand{\dimregion}{{\hc{d}}}
\newcommand{\loc}{{\hc{\bm r}}}
\newcommand{\locx}{{\hc{r}}_{x}}
\newcommand{\normlocx}{{\hc{\check r}}_{x}} % normalized locx
%\newcommand{\locxl}{{\hc{\grave r}}_{x}} % locx lower
%\newcommand{\locxu}{{\hc{\acute r}}_{x}} % locx upper

\newcommand{\locxu}{\stackrel{\lrcorner}{\hc{r}}_x} % locx upper
\newcommand{\locxl}{\stackrel{\llcorner}{\hc{r}}_x} % locx lower

\newcommand{\locy}{{\hc{r}}_{y}}
\newcommand{\locz}{{\hc{r}}_{z}}

\newcommand{\locfull}{{\hc{\underline{\bm r}}}}
\newcommandoa{\srclocfull}{{\hc{\underline{\acute{\bm r}}}}}{{\hc{\underline{\acute{\bm r}}}}_{#1}} % source location
\newcommand{\auxsrclocfull}{{\hc{\underline{\check{\bm r}}}}}
\newcommand{\auxsrclocx}{{\hc{\check r}}_x}
\newcommand{\auxsrclocy}{{\hc{\check r}}_y}
\newcommand{\auxsrclocz}{{\hc{\check r}}_z}

\newcommand{\locfullmeas}{{\hc{\tilde \locfull}}} % location estimate
\newcommand{\locp}{{\hc{\bm r}}'} % loc prime
\newcommand{\locxsp}[1]{{\hc{r}}_{#1}} % locx sampling point
\newcommandoa{\locxspset}{{\hc{\tilde{\mathcal{R}}}}}{{\hc{\tilde{\mathcal{R}}}_{#1}}} % locx sampling point set
\newcommand{\pmapsv}[1]{{\hc{\pmap}}_{#1}} % pmap sampling value
\newcommand{\pmapdelta}[1]{{\hc{\Delta\pmap}}_{#1}} % pmap delta
\newcommand{\pa}[1]{|{\hc{\Delta\pmap}}_{#1}|} % pmap delta abs
\newcommand{\relvar}[1]{\hc{\xi}_{#1}} % relative variation
\newcommand{\relvaropt}[1]{\hc{\xi}_{#1}^*} % optimal relative variation
\newcommand{\locxdelta}[1]{{\hc{\Delta r}}_{#1}} % location delta
\newcommand{\locxmp}[1]{{\hc{\tilde r}}_{#1}} % location mean point
\newcommand{\spind}{{\hc{n}}} % sampling point index
\newcommand{\spnum}{{\hc{N}}} % number of sampling points
\newcommand{\spindset}{{\hc{\mathcal{N}}}} %  index set of sampling points

\newcommand{\ubound}[1]{{\hc{f}}^{(u)}_{#1}} % upper bound
\newcommand{\lbound}[1]{{\hc{f}}^{(l)}_{#1}} % lower bound
\newcommand{\bound}[1]{{\hc{f}}_{#1}} % bound
\newcommand{\cbound}[1]{\hc{\tilde f}_{#1}} % combined bound

\newcommand{\wnx}{{\hc{k}}_{x}} % wavenumber x

\newcommand{\wavelen}{{\hc{\lambda}}} %
%\newcommand{\txpow}{{\hc{P}_\text{Tx}}} %
\newcommandoa{\txpow}{{\hc{P}_\text{Tx}}}{{\hc{P}^{(#1)}_\text{Tx}}} %
\newcommand{\txantgain}{{\hc{G}_\text{Tx}}} %
\newcommand{\rxantgain}{{\hc{G}_\text{Rx}}} % 
\newcommand{\mindist}{{\hc{\eta}}_{\text{min}}} % min distance to apply Friis' equation
\newcommand{\minsrcregdist}{{\hc{d}_{\text{min}}}} % min distance to srcregion

\newcommand{\plane}{{\hc{\mathcal{P}}}} %
%\newcommand{\srcloc}{{\hc{\bbm r}}}

% \newcommand{\srcloc}[1][noargpassed]{% add a subscript if an arg is passed
%   {\hc{\bbm r}}
%   \ifthenelse{\equal{#1}{noargpassed}}{}{_{#1}}%
% }
\newcommandoa{\srcloc}{{\hc{\acute{\bm r}}}}{{\hc{\acute{\bm r}}}_{#1}} % source location
\newcommandoa{\srclocx}{{\hc{\acute r}}_x}{{\hc{\acute{r}}}_{x,#1}} % source location x-coord
\newcommandoa{\srclocy}{{\hc{\acute r}}_y}{{\hc{\acute r}}_{y,#1}} % source location y-coord
\newcommandoa{\srclocz}{{\hc{\acute r}}_z}{{\hc{\acute r}}_{z,#1}} % source location z-coord
\newcommandoa{\rdists}{{\hc{\beta}}^2}{{\hc{\beta}}^2_{#1}} % squared distance to the map region
\newcommandoa{\rdist}{{\hc{\beta}}}{{\hc{\beta}}_{#1}} %  distance to the map region
\newcommand{\auxrdist}{{\hc{b}}}
\newcommandoa{\normrdist}{{\hc{\check \beta}}}{{\hc{\check \beta}}_{#1}} %  normalized distance to the map region
\newcommand{\rdistmin}{{\hc{\beta}}_{\text{min}}} %  minimum distance to the map region
\newcommand{\rdistmax}{{\hc{\beta}}_{\text{max}}} %  maximum distance to the map region
\newcommandoa{\rdistsset}{{\hc{\mathcal{B}}}}





\newcommand{\srcnum}{{\hc{S}}} % number of sources
\newcommand{\srcind}{{\hc{s}}} % index of source
\newcommand{\srcindp}{{\hc{s'}}} % index of source prime
\newcommandoa{\srccoef}{{\hc{\alpha}}}{{\hc{\alpha}}_{#1}} % source coefficient

\newcommand{\prox}{\hc{\rho}} % Proximity factor


\newcommand{\deneps}{{\hc{\eta}}} % small constant for the denominator
\newcommand{\tol}{{\hc{\epsilon}}} % for all epsilon, there exists...

\newcommand{\etfield}{{\hc{\bm e}}} % E field in time
\newcommand{\etsfield}{{\hc{e}}} % E scalar field in time
\newcommand{\effield}{{\hc{\bm E}}} % E field in freq./phasor
\newcommand{\efsfield}{{\hc{E}}} % E scalar field in freq./phasor
\newcommand{\correfield}{{\hc{r_f}}}
\newcommand{\plfield}{{\hc{\gamma}_\text{PL}}}
\newcommand{\shadfield}{{\hc{\gamma}_\text{S}}}
\newcommand{\fadfield}{{\hc{\gamma}_\text{F}}}
\newcommand{\fadbw}{{\hc{W}_\text{F}}}
\newcommand{\shadbw}{{\hc{W}_\text{S}}}
%\newcommand{\volbw}{{\hc{W}_\text{V}}} % bandwidth of the volume

\newcommand{\map}{{\hc{m}}}
\newcommand{\mapest}{{\hc{\hat m}}}

\newcommand{\pmap}{{\hc{\gamma}}} % power map
\newcommand{\pmapval}{{\hc{g}}} % power map value
\newcommand{\pmapvec}{{\hc{\bm \pmap}}} % 
\newcommand{\pmapestvec}{{\hc{\hbm \pmap}}} % 
\newcommand{\pmapoptval}{{\hc{g}^*}} % power map opt val
\newcommand{\normpmap}{{\hc{\check \gamma}}} % normalized arg power map
\newcommand{\pmapest}{{\hc{\hat \gamma}}} % power map estimate
\newcommand{\pmapft}{{\hc{\Gamma}}} % power map Fourier transform
\newcommand{\auxpmap}{{\hc{\bar\gamma}}} % auxiliary power map
\newcommand{\auxpmapt}{{\hc{\check\gamma}}} % auxiliary power map two
\newcommand{\pmapset}{{\hc{\Gamma}}} % power map set
\newcommandoa{\fspmapset}{{\hc{\Gamma_\text{FS}}}}{{\hc{\Gamma_\text{FS}^{(#1)}}}} % free-space power map set [restriction dim]
\newcommandoa{\auxfspmapset}{{\hc{\check\Gamma_\text{FS}}}}{{\hc{\check\Gamma_\text{FS}^{(#1)}}}} % free-space power map set [restriction dim]
\newcommand{\fspmaprdset}[1]{{\hc{\Gamma_\text{FS}^{(#1,\rdists)}}}} % free-space power map rdists set [restriction dim]
\newcommand{\psdmap}{{\hc{\gamma}}}

\newcommand{\hplaneset}{{\hc{\mathcal{H}}}} % horizontal plane
\newcommand{\lineset}{{\hc{\mathcal{L}}}} % line

\newcommand{\deriub}{{\hc{m}}} % derivative upper bound

% \newcommand{\sensnum}{{\hc{L}}} % number of sensors
% \newcommand{\sensind}{{\hc{l}}} % index of sensors
\newcommand{\fmeas}{{\hc{\mathcal{M}}}} % measurement functional
%\newcommand{\meas}{{\hc{\tilde m}}} % measurement
\newcommand{\meas}{\pmap} % measurement
\newcommand{\vecmeas}{{\hc{\bm m}}} % measurement 
\newcommand{\noise}{{\hc{\zeta}}} % measurement noise




\newcommand{\errmet}{{\hc{\mathcal{E}}}} % measurement
\newcommand{\opbl}{{\hc{\mathcal{B}}}} % Bandlimiting operator


\newcommand{\kernel}{{\hc{\kappa}}} % reproducing kernel


\def\timenotation{0}

\if\timenotation1

    \renewcommand{\time}{\hc{t}}
    \newcommand{\sampind}{\hc{n}}
    \newcommand{\sampint}{\hc{T}}
    %\newcommand{\freq}{\hc{t}}
    \newcommand{\sig}{\hc{x}} % signal
    \newcommand{\sigft}{\hc{X}}
    \newcommand{\sigest}{\hc{\hat x}}
    \newcommand{\sigestft}{\hc{\hat X}}
    \newcommand{\shiftsig}{\hc{y}\sigshiftnot{\sigshift}} % shifted signal
    \newcommand{\shiftsigft}{\hc{Y}\sigshiftnot{\sigshift}} % shifted signal FT
    \newcommand{\sigshift}{{\hc{\tau}}} % signal shift
    \newcommand{\sigshiftf}{{\hc{\theta}}} % signal shift fourier dual variable
    \newcommand{\shiftsigest}{\hc{\hat y}\sigshiftnot{\sigshift}} % shifted signal estimate
    \newcommand{\highband}{{\hc{\mathcal{B}}}}

    \newcommand{\auxseq}{\hc{z}} % aux sequence
    \newcommand{\auxseqft}{\hc{Z}} % aux sequence FT
    \newcommand{\freq}{{\hc{\omega}}}

\else


    \renewcommand{\time}{\locx}
    \newcommand{\sampind}{\spind}
    \newcommand{\sampint}{\hc{\locxdelta{}}}
    %\newcommand{\freq}{\hc{t}}
    \newcommand{\sig}{\pmap} % signal
    \newcommand{\sigft}{\pmapft}
    \newcommand{\sigest}{\pmapest}
    \newcommand{\sigestft}{\hat{\pmapft}}
    \newcommand{\sigshift}{{\hc{\nu}}} % signal shift
    \newcommand{\sigshiftf}{{\hc{\theta}}} % signal shift fourier dual variable

    \newcommand{\shiftsig}{\hc{\phi}\sigshiftnot{\sigshift}} % shifted signal
    \newcommand{\shiftsigft}{\hc{\Phi}\sigshiftnot{\sigshift}} % shifted signal FT
    \newcommand{\shiftsigest}{\hc{\hat \phi}\sigshiftnot{\sigshift}} % shifted signal estimate
    \newcommand{\shiftsigestcs}[1]{\hc{\hat \phi}\sigshiftnot{#1}} % shifted signal estimate custom shift
    \newcommand{\auxshiftsigestcs}[1]{\hc{\hat \varphi}\sigshiftnot{#1}} % shifted signal estimate custom shift
    \newcommand{\highband}{{\hc{\mathcal{B}}}}

    \newcommand{\auxseq}{\hc{\psi}} % aux sequence
    \newcommand{\auxseqft}{\hc{\Psi}} % aux sequence FT
    \newcommand{\freq}{\wnx}

\fi


\newcommand{\err}{\hc{E}}
\newcommand{\errp}{\hc{E}'} % error prime
\newcommand{\avgerr}{\hc{\bar E}}
\newcommand{\avgerrp}{\hc{\bar E}'}
\newcommand{\sigshiftnot}[1]{^{(#1)}} % signal shift notation
\newcommand{\compind}{{\hc{m}}}% component index
\newcommand{\rpulse}{\hc{\Pi}} % rectangular pulse


\newcommand{\boundfun}{\hc{c}} % bound function

\newcommand{\radius}{\hc{R}} % bound function

\newcommand{\pathlossexp}{{\hc{\upsilon}}} % path loss exponent
